No Answer is Better Than Wrong Answer: A Reflection Model for Document Level Machine Reading Comprehension

The Natural Questions (NQ) benchmark set brings new challenges to Machine Reading Comprehension: the answers are not only at different levels of granularity (long and short), but also of richer types (including no-answer, yes/no, single-span and multi-span). In this paper, we target at this challenge and handle all answer types systematically. In particular, we propose a novel approach called Reflection Net which leverages a two-step training procedure to identify the no-answer and wrong-answer cases. Extensive experiments are conducted to verify the effectiveness of our approach. At the time of paper writing (May.~20,~2020), our approach achieved the top 1 on both long and short answer leaderboard, with F1 scores of 77.2 and 64.1, respectively.

==> hyperparams_table.tex <==
\begin{table}[htbp]
\resizebox{0.5\textwidth}{!}{%
 \begin{tabular}{l c c c c c } 
 \toprule
   \multirow{2}{*}{\textbf{Hyperparams}} & \multicolumn{2}{c}{BERT} && \multicolumn{2}{c}{RoBERTa} \\
   \cline{2-3}
   \cline{5-6}
    & \textbf{MRC} & \textbf{Reflection} && \textbf{MRC} & \textbf{Reflection}  \\
 \midrule
   Dropout & \multicolumn{2}{c}{0.1} && \multicolumn{2}{c}{0.1}\\
   Attention dropout & \multicolumn{2}{c}{0.1} && \multicolumn{2}{c}{0.1}\\
   Max sequence length & \multicolumn{2}{c}{512} && \multicolumn{2}{c}{512}\\
   Learning Rate &3e-5&5e-6&&2.2e-5&5e-6 \\ 
   Batch Size & \multicolumn{2}{c}{24} && \multicolumn{2}{c}{48}\\
   Weight Decay & \multicolumn{2}{c}{0.01} && \multicolumn{2}{c}{0.01}\\
   Epochs &1&2&&1&2\\
   Learning Rate Decay & \multicolumn{2}{c}{Linear} && \multicolumn{2}{c}{Linear}\\
   Warmup ratio & \multicolumn{2}{c}{0.1} && \multicolumn{2}{c}{0.06}\\
   Gradient Clipping & \multicolumn{2}{c}{1.0} && \multicolumn{2}{c}{-}\\
   Adam $\epsilon$ & \multicolumn{2}{c}{1e-8} && \multicolumn{2}{c}{1e-8}\\
   Adam $\beta_1$ & \multicolumn{2}{c}{0.9} && \multicolumn{2}{c}{0.9}\\
   Adam $\beta_2$ & \multicolumn{2}{c}{0.999} && \multicolumn{2}{c}{0.999}\\
 \bottomrule
\end{tabular}}
\caption{Training hyperparameters of MRC model and Reflection model.}
\label{tab:hyperparameters}
\end{table}

